The worst of both worlds: A comparative analysis of errors in learning from data in psychology and machine learning

Recent arguments that machine learning (ML) is facing a reproducibility and replication crisis suggest that some published claims in ML research cannot be taken at face value. These concerns inspire analogies to the replication crisis affecting the social and medical sciences. They also inspire calls for the integration of statistical approaches to causal inference and predictive modeling. A deeper understanding of what reproducibility concerns in supervised ML research have in common with the replication crisis in experimental science puts the new concerns in perspective, and helps researchers avoid "the worst of both worlds," where ML researchers begin borrowing methodologies from explanatory modeling without understanding their limitations and vice versa. We contribute a comparative analysis of concerns about inductive learning that arise in causal attribution as exemplified in psychology versus predictive modeling as exemplified in ML. We identify themes that re-occur in reform discussions, like overreliance on asymptotic theory and non-credible beliefs about real-world data generating processes. We argue that in both fields, claims from learning are implied to generalize outside the specific environment studied (e.g., the input dataset or subject sample, modeling implementation, etc.) but are often impossible to refute due to undisclosed sources of variance in the learning pipeline. In particular, errors being acknowledged in ML expose cracks in long-held beliefs that optimizing predictive accuracy using huge datasets absolves one from having to consider a true data generating process or formally represent uncertainty in performance claims. We conclude by discussing risks that arise when sources of errors are misdiagnosed and the need to acknowledge the role of human inductive biases in learning and reform.

==> old_2_5_culture.tex <==
\subsection{Culture}
\jessica{considering moving important points from here to discussion and/or background so middle section of paper isn't so long}
\textbf{SP.} 
\jessica{add a summary of the top issues here and to summarize ML section so that they are easier to read/compare}
In accounts seeking to explain the replication crisis, social psychology researchers are described as valuing surprising or counterintuitive effects about human nature [] and emphasizing the power of small interventions to have big effects (e.g., ``nudges'') [], compelled by strong pressures to publish~\cite{fanelli2010pressures} [Fanelli 2010 Do pressures], especially positive evidence~\cite{fanelli2010positive,scargle1999publication}, and the success of simple stylized facts in attracting broad attention to psychology research, such as through pop psychology~\cite{gelman2021did}.

However, these factors can be seen as secondary to an underlying culture in social psychology that accepts ``weak theories'' about mechanisms explaining human behavior in place of those that can make more specific predictions [Meehl, van Rooji etc, others on imprecise theories in psych]. %Without refutable theories, issues with methods, data, and incentives can lead to situations like the replication crisis. 

The influence of behaviorists like Skinner who strove to explain behavior in ways that would encompass all forms of knowledge, from lab rats to scientists themselves~\cite{flis2019psychologists}, allowed psychologists to entertain theories in which certain behavioral traits were innately determined and cognition ``embodied'' [\jessica{TODO: cite something ideally meta analysis or survey on embodied cognition}\PN{What about this book? Shapiro, L. (2010). Embodied cognition. Routledge.}]. However, many theories throughout the literature in social psychology underspecify expected patterns in empirical evidence (i.e., do not specify the expected size of an effect within a narrow range of values~\cite{meehl1990summaries}), such that the theories cannot support concrete, falsifiable predictions [Borsboom 2013] and present challenges to developing cumulative theory~\cite{eronen2021theory}; see also~\cite{oberauer2019addressing,devezer2020case}. Under strong incentives to publish positive evidence of counterintuitive effects and ample flexibility in analysis, this has led to a culture in which experiments are mostly used to confirm hypothesized effects. Together these realities create a situation in which an enhancement of statistical power made by improving the experiment design or measurements or increasing sample size makes it easier for researchers to believe they have confirmed a theory, in direct contrast to how NHST is used to test theories in hard sciences~\cite{meehl1967theory}.

Methodological overconfidence may help explain why psychology at large has not addressed these theoretical weaknesses. 
Despite psychology’s post-WWII move away from algorithmic definitions of rationality toward studying the irrational~\cite{flis2019psychologists}, exemplified for instance by the heuristics and biases regime of the 1970’s (e.g.,~\cite{tversky1974judgment}), experimental methods and the associated machinery for inference have long been treated as a kind of insurance against psychologists’ own biases. In particular, a strong faith in randomized controlled experiments as an unbiased procedure (evidenced, e.g., in the tendency toward between subjects experiments [section ref above]) may lead psychologists to overlook other critical sources of error or uncertainty, like measurement and theory. The tendency to see randomized methods combined with conventional publishing standards like peer review as a form of ``truth mill''~\cite{gelman2014ethics}, such that anything published is seen as synonymous with truth, was explicitly pointed out by reformers starting in the early 2010’s~\cite{nosek2012scientific}. This results in a situation in which beliefs about core methods create a form of hubris in which the scientist's responsibility to refutable theory is overlooked. 

\textbf{ML.} We argue that the cultural root cause of many of the pitfalls and reproducibility failures in ML derives from a similar lack of refutable theory, manifesting in ML as a confusion between engineering artifacts and scientific knowledge. While it is important to improve engineering practices and heuristics about ML models to better understand which models work better under what contexts, especially from the viewpoint of improving products and services that use ML, for progress to continue, scientific knowledge needs to be generalizable in ways that current reliance on heuristics and ``possibilistic'' accuracy claims prevent.

%. The pervasiveness of heuristics about ML models in the current culture stand in the way of creating generalizable knowledge.

Consider a typical ML paper that provides an innovative algorithm, architecture, or model and shows that it achieves a certain accuracy on a benchmark dataset. % (it is common to compare to multiple existing algorithms and claim to beat the state of the art, and somewhat common to consider multiple benchmarks, but this doesn’t change our analysis). 
Even if we assume the reported accuracy is not optimistic for the reasons discussed above, the researcher has contributed an engineering artifact, a tool that the practicing engineer can carry in their toolbox: the algorithm or model for which performance has been found superior to the state-of-the-art on a particular learning problem.  %They don't know a priori how well the tool will work in a new scenario, but they can try different tools from their toolbox and pick the best one for the job. 
New observations based on additional data cannot refute the performance claim of the given algorithm on the given dataset, because the population from which benchmark datasets are drawn are rarely specified to the detail needed for another sample to be drawn~\cite{jo2020lessons}.
%If the dataset were a sample from a population, a different researcher could collect a different sample from the population and attempt to refute the claim. Unfortunately, in ML praxis, the population from which  
Attempts to collect a different sample from an implied population to try to refute claims are extremely rare; when they have been attempted, researchers have found that the original claims no longer hold on the new samples~\cite{recht2019unbiased}. Further, when researchers have tried to compare model performance across benchmark datasets, they have found that results on one benchmark rarely generalize to another, and can be extremely fragile~\cite{torralba2011unbiased,dehghani2021benchmark}.
%. But engineering is different from science. Although the philosophy of science is a vast field and views vary, 


At a higher level, analogies between human and artificial intelligence are embedded in AI and ML culture, but similarly atheoretical in most forms. 
These occur through post-hoc rationalization that ML approaches are capturing critical aspects of human consciousness (e.g.,~\cite{}) and descriptions of new algorithms as inspired by human cognition (e.g.,~\cite{bengio2017consciousness}). Without a priori specification of what humans do or how  to explain the implementation of high level cognitive
algorithms that are of interest in AI in terms of
neurocomputational processing~\cite{reggia2020artificial}, the field remains unable to validate whether algorithms meant to accomplish human-like tasks have succeeded in a human-like way (see also Section~\ref{}). 


The acceptance of non-refutable research claims as research contributions, much as in social psychology, creates a culture in which other methodological issues amplify the difficulty of building generalizable knowledge. 
%Engineering knowledge and artifacts are valid and valuable. 
%While producing engineering knowledge is an important step towards developing a better "toolbox" for practitioners, and indeed can help improve the performance of ML models on real world tasks, a core tenet of science is improving understanding of the world via falsifiable claims. However in the typical ML paper we described, 
If not recognized and addressed, hubris that big data renders typical requirements in statistical modeling like uncertainty quantification~\cite{dehghani2021benchmark}[Bouthillier 2021, Lin 2021 (arxiv)] unnecessary, combined with a general lack of rigor in evaluation~\cite{sculley2018winner,liao2021we} and overreliance on theory~\cite{lipton2019research} [Goldstein 2022 talk] might leave ML in a similar longterm situation as social psychology, which remains plagued with issues associated with the replication crisis.   
%We hope that our paper shows a path toward a more scientifically grounded approach to machine learning research.

More generally, implications of the prioritization of abstraction to enable scale in ML culture are increasingly questioned. 
Datasets that are ``universal'' are prioritized over those that are more contextual and specific to the task at hand~\cite{scheuerman2021datasets}, leading to a limited number of datasets that tend to be created by a few large institutions [Koch '21]. Further, ML models are often tested on datasets that are built for a completely different application than the task at hand [Koch '21 NeurIPS]. This focus on abstraction and universality in the service of scale leads to the field prioritizing research that is removed from the underlying domain of interest. Consequently, ML models created by researchers can often be inconsistent with best practices in the domain of interest, and as a result, cannot be used in that domain (e.g.,~\cite{nagendran2020artificial,roberts2021common}). 

Just as chasing state-of-the-art (SOTA) performance on benchmark datasets offers researchers a perverse incentive to "cheat", once adopted as a standard across an entire field, the use of benchmarks can replace broader research directions and instead focus the attention of the entire field on improving performance on a limited number of datasets~\cite{raji2021ai,sculley2018winner}. Hypothesis driven scientific inquiry is replaced by incremental improvements to the performance on a limited number of datasets~\cite{hooker1995testing}. As a result, new research questions and directions are ignored in favor of benchmark performance. This issue is exacerbated due to the sudden increase in the size of the field and the requirement for an increasing number of well-trained reviewers and the lack of familiarity of reviewers with the vast amount of literature recently introduced in the field [Church 2022]—in the absence of deep expertise on the subject matter of a paper, an improvement in benchmark performance provides a heuristic to judge the contributions of the paper.
